A Systematic Literature Review on Model-driven Engineering for Cyber-Physical Systems

This technical report presents a Systematic Literature Review (SLR) study that focuses on identifying and classifying the recent research practices pertaining to CPS development through MDE approaches. The study evaluates 140 research papers published during 2010-2018. Accordingly, a comprehensive analysis of various MDE approaches used in the development life-cycle of CPS is presented. Furthermore, the study identifies the research gaps and areas that need more investigation. The contribution helps researchers and practitioners to get an overall understanding of the research trends and existing challenges for further research/development.

==> PrimaryStudiesBib <==
@inproceedings{Angelo2018,
  title={CyPhEF: a model-driven engineering framework for self-adaptive cyber-physical systems},
  author={Angelo, Mirko and Napolitano, Annalisa and Caporuscio, Mauro},
  booktitle={Proceedings of the 40th International Conference on Software Engineering: Companion Proceeedings},
  pages={101--104},
  year={2018},
  organization={ACM}
}

@inproceedings{Aziz2016,
  title={Domain specific modeling language for cyber physical systems},
  author={Aziz, Muhammad Waqar and Rashid, Muhammad},
  booktitle={2016 International Conference on Information Systems Engineering (ICISE)},
  pages={29--33},
  year={2016},
  organization={IEEE}
}

@inproceedings{Ataide2018,
  title={Towards automatic code generation for distributed cyber-physical systems: A first prototype for Arduino boards},
  author={Ata{\'\i}de, Artur and Barros, Jo{\~a}o Paulo and Brito, Isabel Sofia and Gomes, Lu{\'\i}s},
  booktitle={2017 22nd IEEE International Conference on Emerging Technologies and Factory Automation (ETFA)},
  pages={1--4},
  year={2017},
  organization={IEEE}
}

@incollection{Son2012a,
  title={Metamodel design for model transformation from Simulink to ECML in cyber physical systems},
  author={Son, Hyun Seung and Kim, Woo Yeol and Kim, Robert YoungChul and Min, Hang-Gi},
  booktitle={Computer Applications for Graphics, Grid Computing, and Industrial Environment},
  pages={56--60},
  year={2012},
  publisher={Springer}
}

@inproceedings{Alrimawi2018,
  title={I've seen this before: sharing cyber-physical incident knowledge},
  author={Alrimawi, Faeq and Pasquale, Liliana and Mehta, Deepak and Nuseibeh, Bashar},
  booktitle={2018 IEEE/ACM 1st International Workshop on Security Awareness from Design to Deployment (SEAD)},
  pages={33--40},
  year={2018},
  organization={IEEE}
}

@inproceedings{Tariq2012,
  title={Model-driven performance analysis of large scale irrigation networks},
  author={Tariq, Muhammad Umer and Nasir, Hasan Arshad and Muhammad, Abubakr and Wolf, Marilyn},
  booktitle={2012 IEEE/ACM Third International Conference on Cyber-Physical Systems},
  pages={151--160},
  year={2012},
  organization={IEEE}
}

@inproceedings{Guo2018,
  title={Model and integrate medical resource available times and relationships in verifiably correct executable medical best practice guideline models},
  author={Guo, Chunhui and Fu, Zhicheng and Zhang, Zhenyu and Ren, Shangping and Sha, Lui},
  booktitle={Proceedings of the 9th ACM/IEEE International Conference on Cyber-Physical Systems},
  pages={253--262},
  year={2018},
  organization={IEEE Press}
}

@inproceedings{Peters2015,
  title={A generic representation of CCSL time constraints for UML/MARTE models},
  author={Peters, Judith and Wille, Robert and Przigoda, Nils and K{\"u}hne, Ulrich and Drechsler, Rolf},
  booktitle={Proceedings of the 52nd Annual Design Automation Conference},
  pages={122},
  year={2015},
  organization={ACM}
}

@inproceedings{Martins2015,
  title={Towards a systematic threat modeling approach for cyber-physical systems},
  author={Martins, Goncalo and Bhatia, Sajal and Koutsoukos, Xenofon and Stouffer, Keith and Tang, CheeYee and Candell, Richard},
  booktitle={2015 Resilience Week (RWS)},
  pages={1--6},
  year={2015},
  organization={IEEE}
}

@inproceedings{Garamvolgyi2018,
  title={Towards Model-Driven Engineering of Smart Contracts for Cyber-Physical Systems},
  author={Garamv{\"o}lgyi, P{\'e}ter and Kocsis, Imre and Gehl, Benj{\'a}min and Klenik, Attila},
  booktitle={2018 48th Annual IEEE/IFIP International Conference on Dependable Systems and Networks Workshops (DSN-W)},
  pages={134--139},
  year={2018},
  organization={IEEE}
}

@inproceedings{Walch2017a,
  title={Knowledge-driven enrichment of cyber-physical systems for industrial applications using the KbR modelling approach},
  author={Walch, Michael},
  booktitle={2017 IEEE International Conference on Agents (ICA)},
  pages={84--89},
  year={2017},
  organization={IEEE}
}

@inproceedings{Nikiforova2017a,
  title={The two-hemisphere modelling approach to the composition of cyber-physical systems},
  author={Nikiforova, Oksana and El Marzouki, Nisrine and Gusarovs, Konstantins and Vangheluwe, Hans and Bures, Tomas and Al-Ali, Rima and Iacono, Mauro and Esquivel, Priscill Orue and Leon, Florin},
  booktitle={12th International Conference on Software Technologies, ICSOFT 2017},
  pages={286--293},
  year={2017},
  organization={SciTePress}
}

@inproceedings{Nagele2017,
  title={Rapid Construction of Co-simulations of Cyber-Physical Systems in HLA using a DSL},
  author={N{\"a}gele, Thomas and Hooman, Jozef},
  booktitle={2017 43rd Euromicro Conference on Software Engineering and Advanced Applications (SEAA)},
  pages={247--251},
  year={2017},
  organization={IEEE}
}

@inproceedings{Maksuti2017,
  title={Towards flexible and secure end-to-end communication in industry 4.0},
  author={Maksuti, Silia and Bicaku, Ani and Tauber, Markus and Palkovits-Rauter, Silke and Haas, Sarah and Delsing, Jerker},
  booktitle={2017 IEEE 15th International Conference on Industrial Informatics (INDIN)},
  pages={883--888},
  year={2017},
  organization={IEEE}
}

@inproceedings{Goncalves2016a,
  title={Model driven engineering approach to design sensing and actuation subsystems},
  author={Gon{\c{c}}alves, Fernando Silvano and Becker, Leandro Buss},
  booktitle={2016 IEEE 21st International Conference on Emerging Technologies and Factory Automation (ETFA)},
  pages={1--8},
  year={2016},
  organization={IEEE}
}

@inproceedings{Mamun2013,
  title={MDE-based sensor management and verification for a self-driving miniature vehicle},
  author={Mamun, Md Abdullah Al and Berger, Christian and Hansson, Jorgen},
  booktitle={Proceedings of the 2013 ACM workshop on Domain-specific modeling},
  pages={1--6},
  year={2013},
  organization={ACM}
}

@inproceedings{Latombe2015a,
  title={Weaving concurrency in executable domain-specific modeling languages},
  author={Latombe, Florent and Cr{\'e}gut, Xavier and Combemale, Beno{\^\i}t and Deantoni, Julien and Pantel, Marc},
  booktitle={Proceedings of the 2015 ACM SIGPLAN International Conference on Software Language Engineering},
  pages={125--136},
  year={2015},
  organization={ACM}
}

@inproceedings{Merschak2018,
  title={A Hierarchical Meta-Model for the Design of Cyber-Physical Production Systems},
  author={Merschak, Simon and Hehenberger, Peter and Witters, Maarten and Gadeyne, Klaas},
  booktitle={2018 19th International Conference on Research and Education in Mechatronics (REM)},
  pages={36--41},
  year={2018},
  organization={IEEE}
}

@inproceedings{Gerking2015,
  title={Domain-Specific Model Checking for Cyber-Physical Systems},
  author={Gerking, Christopher and Schafer, Wilhelm and Dziwok, Stefan and Heinzemann, Christian},
  booktitle={MoDeVVa\@MoDELS},
  pages={18--27},
  year={2015}
}

@inproceedings{Cicirelli2016,
  title={A meta-model framework for the design and analysis of smart cyber-physical environments},
  author={Cicirelli, Franco and Fortino, Giancarlo and Guerrieri, Antonio and Spezzano, Giandomenico and Vinci, Andrea},
  booktitle={2016 IEEE 20th International Conference on Computer Supported Cooperative Work in Design (CSCWD)},
  pages={687--692},
  year={2016},
  organization={IEEE}
}

@inproceedings{Zhou2018,
  title={Verifying CPS for Self-Adaptability},
  author={Zhou, Ying and Gong, Xufang and Li, Jiakai and Li, Bixin},
  booktitle={2018 IEEE/ACIS 17th International Conference on Computer and Information Science (ICIS)},
  pages={166--172},
  year={2018},
  organization={IEEE}
}

@inproceedings{Zhang2013a,
  title={View Oriented Approach to Specify and Model Aerospace Cyber-physical Systems},
  author={Zhang, Lichen},
  booktitle={2013 IEEE 11th International Conference on Dependable, Autonomic and Secure Computing},
  pages={296--303},
  year={2013},
  organization={IEEE}
}

@inproceedings{Zhang2013b,
  title={Model-based software synthesis for self-reconfigurable sensor network in water monitoring},
  author={Zhang, Kun and Sprinkle, Jonathan},
  booktitle={2013 20th IEEE International Conference and Workshops on Engineering of Computer Based Systems (ECBS)},
  pages={40--48},
  year={2013},
  organization={IEEE}
}

@article{Koutsoukos2012,
  title={A passivity approach for model-based compositional design of networked control systems},
  author={Koutsoukos, Xenofon and Kottenstette, Nicholas and Hall, Joseph and Eyisi, Emeka and Leblanc, Heath and Porter, Joseph and Sztipanovits, Janos},
  journal={ACM Transactions on Embedded Computing Systems (TECS)},
  volume={11},
  number={4},
  pages={75},
  year={2012},
  publisher={ACM}
}

@inproceedings{Drago2013,
  title={Model-driven estimation of distributed vulnerability in complex railway networks},
  author={Drago, Annarita and Marrone, Stefano and Mazzocca, Nicola and Tedesco, Annarita and Vittorini, Valeria},
  booktitle={2013 IEEE 10th International Conference on Ubiquitous Intelligence and Computing and 2013 IEEE 10th International Conference on Autonomic and Trusted Computing},
  pages={380--387},
  year={2013},
  organization={IEEE}
}

@incollection{Jeon2012,
  title={Metamodel-based cps modeling tool},
  author={Jeon, Jaeho and Chun, InGeol and Kim, WonTae},
  booktitle={Embedded and Multimedia Computing Technology and Service},
  pages={285--291},
  year={2012},
  publisher={Springer}
}

@inproceedings{Buckl2010,
  title={FTOS: Model-driven development of fault-tolerant automation systems},
  author={Buckl, Christian and Sojer, Dominik and Knoll, Alois},
  booktitle={2010 IEEE 15th Conference on Emerging Technologies \& Factory Automation (ETFA 2010)},
  pages={1--8},
  year={2010},
  organization={IEEE}
}

@article{Silva2015,
  title={A model-based approach to support validation of medical cyber-physical systems},
  author={Silva, Lenardo and Almeida, Hyggo and Perkusich, Angelo and Perkusich, Mirko},
  journal={Sensors},
  volume={15},
  number={11},
  pages={27625--27670},
  year={2015},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@inproceedings{Bao2016,
  title={Reasoning for cps education using surrogate simulation models},
  author={Bao, Shunxing and Porter, Joe and Gokhale, Aniruddha},
  booktitle={2016 IEEE 40th Annual Computer Software and Applications Conference (COMPSAC)},
  volume={1},
  pages={764--773},
  year={2016},
  organization={IEEE}
}

@inproceedings{Simko2013a,
  title={A framework for unambiguous and extensible specification of DSMLs for cyber-physical systems},
  author={Simko, Gabor and Lindecker, David and Levendovszky, Tihamer and Jackson, Ethan and Neema, Sandeep and Sztipanovits, Janos},
  booktitle={2013 20th IEEE International Conference and Workshops on Engineering of Computer Based Systems (ECBS)},
  pages={30--39},
  year={2013},
  organization={IEEE}
}

@inproceedings{Chen2017,
  title={A model-based approach to dynamic self-assessment for automated performance and safety awareness of cyber-physical systems},
  author={Chen, DeJiu and Lu, Zhonghai},
  booktitle={International Symposium on Model-Based Safety and Assessment},
  pages={227--240},
  year={2017},
  organization={Springer}
}

@inproceedings{Sapienza2014,
  title={Architectural decisions for HW/SW partitioning based on multiple extra-functional properties},
  author={Sapienza, Gaetana and Crnkovic, Ivica and Potena, Pasqualina},
  booktitle={2014 IEEE/IFIP Conference on Software Architecture},
  pages={175--184},
  year={2014},
  organization={IEEE}
}

@article{Housh2018,
  title={Model-based approach for cyber-physical attack detection in water distribution systems},
  author={Housh, Mashor and Ohar, Ziv},
  journal={Water research},
  volume={139},
  pages={132--143},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{Bougouffa2018,
  title={Industry 4.0 interface for dynamic reconfiguration of an open lab size automated production system to allow remote community experiments},
  author={Bougouffa, Safa and Me{\ss}zmer, K and Cha, Suhyun and Trunzer, Emanuel and Vogel-Heuser, Birgit},
  booktitle={2017 IEEE International Conference on Industrial Engineering and Engineering Management (IEEM)},
  pages={2058--2062},
  year={2017},
  organization={IEEE}
}

@inproceedings{Zhang2014,
  title={A closed-loop model-based design approach based on automatic verification and transformation},
  author={Zhang, Kun and Sprinkle, Jonathan},
  booktitle={Proceedings of the 14th Workshop on Domain-Specific Modeling},
  pages={1--6},
  year={2014},
  organization={ACM}
}

@article{Cicirelli2017a,
  title={Metamodeling of smart environments: from design to implementation},
  author={Cicirelli, Franco and Fortino, Giancarlo and Guerrieri, Antonio and Spezzano, Giandomenico and Vinci, Andrea},
  journal={Advanced Engineering Informatics},
  volume={33},
  pages={274--284},
  year={2017},
  publisher={Elsevier}
}

@incollection{Lynch2016,
  title={Ontology-driven metamodel validation in cyber-physical systems},
  author={Lynch, Kevin and Ramsey, Randall and Ball, George and Schmit, Matt and Collins, Kyle},
  booktitle={Information Technology: New Generations},
  pages={1255--1258},
  year={2016},
  publisher={Springer}
}

@inproceedings{Qian2013,
  title={A TAOPN approach to modeling and scheduling cyber-physical systems},
  author={Qian, Zhilin and Yu, Huiqun},
  booktitle={2013 International Conference on Information Science and Applications (ICISA)},
  pages={1--7},
  year={2013},
  organization={IEEE}
}

@inproceedings{Zhang2013c,
  title={An integration approach to specify and model automotive cyber physical systems},
  author={Zhang, Lichen},
  booktitle={2013 International Conference on Connected Vehicles and Expo (ICCVE)},
  pages={568--573},
  year={2013},
  organization={IEEE}
}

@article{Matinnejad2018,
  title={Test generation and test prioritization for simulink models with dynamic behavior},
  author={Matinnejad, Reza and Nejati, Shiva and Briand, Lionel and Bruckmann, Thomas},
  journal={IEEE Transactions on Software Engineering},
  year={2018},
  publisher={IEEE}
}

@article{Thramboulidis2018,
  title={Towards an IoT-based framework for evolvable assembly systems},
  author={Thramboulidis, Kleanthis and Kontou, Ioanna and Vachtsevanou, Danai C},
  journal={IFAC-PapersOnLine},
  volume={51},
  number={11},
  pages={182--187},
  year={2018},
  publisher={Elsevier}
}

@article{Liu2017a,
  title={Modeling cyber-physical attacks based on probabilistic colored Petri nets and mixed-strategy game theory},
  author={Liu, Xiaoxue and Zhang, Jiexin and Zhu, Peidong},
  journal={International Journal of Critical Infrastructure Protection},
  volume={16},
  pages={13--25},
  year={2017},
  publisher={Elsevier}
}

@inproceedings{Guo2017,
  title={Pattern-based statechart modeling approach for medical best practice guidelines-a case study},
  author={Guo, Chunhui and Fu, Zhicheng and Ren, Shangping and Jiang, Yu and Rahmaniheris, Maryam and Sha, Lui},
  booktitle={2017 IEEE 30th International Symposium on Computer-Based Medical Systems (CBMS)},
  pages={117--122},
  year={2017},
  organization={IEEE}
}

@article{Gritzner2018,
  title={Generating correct, compact, and efficient PLC Code from scenario-based assume-guarantee specifications},
  author={Gritzner, Daniel and Greenyer, Joel},
  journal={Procedia Manufacturing 24 (2018)},
  volume={24},
  pages={153--158},
  year={2018},
  publisher={Amsterdam: Elsevier BV}
}

@inproceedings{DiNatale2016,
  title={Matching execution architecture models with functional models to analyze the time performance of CPS systems},
  author={Di Natale, Marco and Morelli, Matteo and Cremona, Fabio},
  booktitle={2015 International Conference on Complex Systems Engineering (ICCSE)},
  pages={1--6},
  year={2015},
  organization={IEEE}
}

@inproceedings{Pajic2012,
  title={From verification to implementation: A model translation tool and a pacemaker case study},
  author={Pajic, Miroslav and Jiang, Zhihao and Lee, Insup and Sokolsky, Oleg and Mangharam, Rahul},
  booktitle={2012 IEEE 18th Real Time and Embedded Technology and Applications Symposium},
  pages={173--184},
  year={2012},
  organization={IEEE}
}

@inproceedings{Cheh2017,
  title={Developing models for physical attacks in cyber-physical systems},
  author={Cheh, Carmen and Keefe, Ken and Feddersen, Brett and Chen, Binbin and Temple, William G and Sanders, William H},
  booktitle={Proceedings of the 2017 Workshop on Cyber-Physical Systems Security and PrivaCy},
  pages={49--55},
  year={2017},
  organization={ACM}
}

@inproceedings{Brito2017,
  title={From requirements to code (Re2Code)—A model-based approach for controller implementation},
  author={Brito, Isabel Sofia and Barros, Jo{\~a}o Paulo and Gomes, Lu{\'\i}s},
  booktitle={2016 IEEE 14th International Conference on Industrial Informatics (INDIN)},
  pages={1224--1230},
  year={2016},
  organization={IEEE}
}

@inproceedings{Chen2016,
  title={A model-based approach to qualified process automation for anomaly detection and treatment},
  author={Chen, DeJiu and Panfilenko, Dmitri Valeri and Khabbazi, Mahmood R and Sonntag, Daniel},
  booktitle={2016 IEEE 21st International Conference on Emerging Technologies and Factory Automation (ETFA)},
  pages={1--8},
  year={2016},
  organization={IEEE}
}

@inproceedings{Kothari2018,
  title={Modeling lessons from verifying large software systems for safety and security},
  author={Kothari, Suresh and Awadhutkar, Payas and Tamrawi, Ahmed and Mathews, Jon},
  booktitle={Proceedings of the 2017 Winter Simulation Conference},
  pages={109},
  year={2017},
  organization={IEEE Press}
}

@inproceedings{Neema2014,
  title={Formalization of software models for cyber-physical systems},
  author={Neema, Sandeep and Simko, Gabor and Levendovszky, Tihamer and Porter, Joseph and Agrawal, Akshay and Sztipanovits, Janos},
  booktitle={Proceedings of the 2nd FME Workshop on Formal Methods in Software Engineering},
  pages={45--51},
  year={2014},
  organization={ACM}
}

@inproceedings{Zhang2014c,
  title={A framework to specify big data driven complex cyber physical control systems},
  author={Zhang, Lichen},
  booktitle={2014 IEEE International Conference on Information and Automation (ICIA)},
  pages={548--553},
  year={2014},
  organization={IEEE}
}

@inproceedings{Parveen2018,
  title={Design and feasibility study of health related devices using COTS components},
  author={Parveen, Rizwan and Pradhan, Shubham and Goveas, Neena},
  booktitle={2018 IEEE Industrial Cyber-Physical Systems (ICPS)},
  pages={529--533},
  year={2018},
  organization={IEEE}
}

@inproceedings{Zhang2014d,
  title={Integration design and model transformation for cyber physical systems},
  author={Zhang, Lichen and Feng, Shuguang},
  booktitle={2014 IEEE 5th International Conference on Software Engineering and Service Science},
  pages={754--757},
  year={2014},
  organization={IEEE}
}

@article{Jiang2018,
  title={Dependable model-driven development of cps: From stateflow simulation to verified implementation},
  author={Jiang, Yu and Song, Houbing and Yang, Yixiao and Liu, Han and Gu, Ming and Guan, Yong and Sun, Jiaguang and Sha, Lui},
  journal={ACM Transactions on Cyber-Physical Systems},
  volume={3},
  number={1},
  pages={12},
  year={2019},
  publisher={ACM}
}

@inproceedings{Pereira2016,
  title={The IOPT-Flow framework pairing Petri nets and data-flows for embedded controller development},
  author={Pereira, Fernando and Gomes, Lu{\'\i}s},
  booktitle={IECON 2016-42nd Annual Conference of the IEEE Industrial Electronics Society},
  pages={4832--4837},
  year={2016},
  organization={IEEE}
}

@inproceedings{Mezhuyev2013,
  title={Geometrical meta-metamodel for cyber-physical modelling},
  author={Mezhuyev, Vitaliy and Samet, Refik},
  booktitle={2013 International Conference on Cyberworlds},
  pages={89--93},
  year={2013},
  organization={IEEE}
}

@article{Ollinger2013,
  title={An integrated concept for the model-driven engineering of distributed automation architectures on embedded systems},
  author={Ollinger, Lisa and Wehrmeister, Marco A and Pereira, Carlos E and Z{\"u}hlke, Detlef},
  journal={IFAC Proceedings Volumes},
  volume={46},
  number={7},
  pages={222--227},
  year={2013},
  publisher={Elsevier}
}

@inproceedings{Huang2018,
  title={Towards modeling cyber-physical systems with SysML/MARTE/pCCSL},
  author={Huang, Ping and Jiang, Kaiqiang and Guan, Chunlin and Du, Dehui},
  booktitle={2018 IEEE 42nd Annual Computer Software and Applications Conference (COMPSAC)},
  volume={1},
  pages={264--269},
  year={2018},
  organization={IEEE}
}

@article{Lavigne2018,
  title={AVS, a model-based racing sailboat simulator: application to wind integration},
  author={Lavigne, Emilien and Guillou, Goulven and Babau, Jean-Philippe},
  journal={IFAC-PapersOnLine},
  volume={51},
  number={10},
  pages={88--94},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{Goncalves2017,
  title={Formal Verification of AADL Models Using UPPAAL},
  author={Gon{\c{c}}alves, Fernando Silvano and Pereira, David and Tovar, Eduardo and Becker, Leandro Buss},
  booktitle={2017 VII Brazilian Symposium on Computing Systems Engineering (SBESC)},
  pages={117--124},
  year={2017},
  organization={IEEE}
}

@article{Chen2015,
  title={A virtual environment for the management and development of cyber-physical manufacturing systems},
  author={Chen, DeJiu and Maffei, Antonio and Ferreirar, Jo{\~a}o and Akillioglu, Hakan and Khabazzi, Mahmood R and Zhang, Xinhai},
  journal={IFAC-PapersOnLine},
  volume={48},
  number={7},
  pages={29--36},
  year={2015},
  publisher={Elsevier}
}

@article{Weissnegger2016a,
  title={Simulation-based verification of automotive safety-critical systems based on EAST-ADL},
  author={Weissnegger, Ralph and Schuss, Markus and Kreiner, Christian and Pistauer, Markus and R{\"o}mer, Kay and Steger, Christian},
  journal={Procedia computer science},
  volume={83},
  pages={245--252},
  year={2016},
  publisher={Elsevier}
}

@inproceedings{Tariq2014,
  title={Design Specification of Cyber-Physical Systems: Towards a Domain-Specific Modeling Language based on Simulink, Eclipse Modeling Framework, and Giotto.},
  author={Tariq, Muhammad Umer and Florence, Jacques and Wolf, Marilyn},
  booktitle={ACESMB@ MoDELS},
  pages={6--15},
  year={2014}
}

@article{Mordecai2018,
  title={Conceptual Modeling of Cyber-Physical Gaps in Air Traffic Control},
  author={Mordecai, Yaniv},
  journal={Procedia Computer Science},
  volume={140},
  pages={21--28},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{Bunting2016,
  title={A safe autonomous vehicle trajectory domain specific modeling language for non-expert development},
  author={Bunting, Matt and Zeleke, Yegeta and McKeever, Kennon and Sprinkle, Jonathan},
  booktitle={Proceedings of the International Workshop on Domain-Specific Modeling},
  pages={42--48},
  year={2016},
  organization={ACM}
}

@inproceedings{Hartmann2015,
  title={Stream my models: Reactive peer-to-peer distributed models@ run. time},
  author={Hartmann, Thomas and Moawad, Assaad and Fouquet, Fran{\c{c}}ois and Nain, Gr{\'e}gory and Klein, Jacques and Le Traon, Yves},
  booktitle={2015 ACM/IEEE 18th International Conference on Model Driven Engineering Languages and Systems (MODELS)},
  pages={80--89},
  year={2015},
  organization={IEEE}
}

@inproceedings{Banerjee2014,
  title={Model based code generation for medical cyber physical systems},
  author={Banerjee, Ayan and Gupta, Sandeep KS},
  booktitle={Proceedings of the 1st Workshop on Mobile Medical Applications},
  pages={22--27},
  year={2014},
  organization={ACM}
}

@inproceedings{Liu2011,
  title={Aspect-Oriented MDA Development Method for Non-Functional Properties of Cyber Physical Systems},
  author={Liu, Jingyong and Zhang, Lichen},
  booktitle={2011 Second International Conference on Networking and Distributed Computing},
  pages={149--153},
  year={2011},
  organization={IEEE}
}

@inproceedings{Sanislav2017,
  title={A dependability analysis model in the context of cyber-physical systems},
  author={Sanislav, Teodora and Mois, George},
  booktitle={2017 18th International Carpathian Control Conference (ICCC)},
  pages={146--150},
  year={2017},
  organization={IEEE}
}

@inproceedings{Lora2017,
  title={Virtual prototyping of smart systems through automatic abstraction and mixed-signal scheduling},
  author={Lora, Michele and Fraccaroli, Enrico and Fummi, Franco},
  booktitle={2017 22nd Asia and South Pacific Design Automation Conference (ASP-DAC)},
  pages={232--237},
  year={2017},
  organization={IEEE}
}

@inproceedings{An2011,
  title={Model-driven performance analysis of reconfigurable conveyor systems used in material handling applications},
  author={An, Kyoungho and Trewyn, Adam and Gokhale, Aniruddha and Sastry, Shivakumar},
  booktitle={2011 IEEE/ACM Second International Conference on Cyber-Physical Systems},
  pages={141--150},
  year={2011},
  organization={IEEE}
}

@inproceedings{Motii2017,
  title={Guiding the selection of security patterns for real-time systems},
  author={Motii, Anas and Hamid, Brahim and Lanusse, Agnes and Bruel, Jean-Michel},
  booktitle={2016 21st International Conference on Engineering of Complex Computer Systems (ICECCS)},
  pages={155--164},
  year={2016},
  organization={IEEE}
}

@inproceedings{VanDeMortel-Fronczak2014,
  title={Supervisor synthesis in model-based automotive systems engineering},
  author={Van Mortel-Fronczak, Joanna M and van der Heijden, Martin HR and Huisman, Rudolf GM and Reniers, Michel A},
  booktitle={ICCPS'14: ACM/IEEE 5th International Conference on Cyber-Physical Systems (with CPS Week 2014)},
  pages={187--198},
  year={2014},
  organization={IEEE Computer Society}
}

@article{Li2015,
  title={CPSiCGF: A code generation framework for CPS integration modeling},
  author={Li, Song and Li, Di and Li, Fang and Zhou, Nan},
  journal={Microprocessors and Microsystems},
  volume={39},
  number={8},
  pages={1234--1244},
  year={2015},
  publisher={Elsevier}
}

@inproceedings{He2018,
  title={Modeling and Analyzing Cyber Physical Systems Using High Level Petri Nets},
  author={He, Xudong},
  booktitle={2018 IEEE International Conference on Software Quality, Reliability and Security Companion (QRS-C)},
  pages={469--476},
  year={2018},
  organization={IEEE}
}

@inproceedings{Whitsitt2014,
  title={Generating model transformations for mending dynamic constraint violations in cyber physical systems},
  author={Whitsitt, Sean and Sprinkle, Jonathan and Lysecky, Roman},
  booktitle={Proceedings of the 14th Workshop on Domain-Specific Modeling},
  pages={35--40},
  year={2014},
  organization={ACM}
}

@inproceedings{Bocciarelli2017,
  title={A BPMN extension for modeling Cyber-Physical-Production-Systems in the context of Industry 4.0},
  author={Bocciarelli, Paolo and D'Ambrogio, Andrea and Giglio, Andrea and Paglia, Emiliano},
  booktitle={2017 IEEE 14th International Conference on Networking, Sensing and Control (ICNSC)},
  pages={599--604},
  year={2017},
  organization={IEEE}
}

@article{Seiger2015,
  title={Modelling complex and flexible processes for smart cyber-physical environments},
  author={Seiger, Ronny and Keller, Christine and Niebling, Florian and Schlegel, Thomas},
  journal={Journal of Computational Science},
  volume={10},
  pages={137--148},
  year={2015},
  publisher={Elsevier}
}

@inproceedings{Tuo2017,
  title={An Approach for Safety Analysis of Cyber-Physical System Based on Model Transformation},
  author={Tuo, Mingfu and Zhou, Xingshe and Yang, Gang and Fu, Ning},
  booktitle={2016 IEEE International Conference on Internet of Things (iThings) and IEEE Green Computing and Communications (GreenCom) and IEEE Cyber, Physical and Social Computing (CPSCom) and IEEE Smart Data (SmartData)},
  pages={636--639},
  year={2016},
  organization={IEEE}
}

@inproceedings{Tundis2017,
  title={Applying a properties modeling approach for monitoring smart grids},
  author={Tundis, Andrea and Egert, Rolf and M{\"u}hlh{\"a}user, Max},
  booktitle={2017 IEEE 14th International Conference on Networking, Sensing and Control (ICNSC)},
  pages={714--719},
  year={2017},
  organization={IEEE}
}

@inproceedings{Ciavotta2018,
  title={Interoperable meta model for simulation-in-the-loop},
  author={Ciavotta, Michele and Bettoni, Andrea and Izzo, Gabriele},
  booktitle={2018 IEEE Industrial Cyber-Physical Systems (ICPS)},
  pages={702--707},
  year={2018},
  organization={IEEE}
}

@inproceedings{Dell2014,
  title={Model-based platform design and evaluation of cloud-based cyber-physical systems (CCPS)},
  author={Dell, Johannes and Greiner, Thomas and Rosenstiel, Wolfgang},
  booktitle={2014 12th IEEE International Conference on Industrial Informatics (INDIN)},
  pages={376--381},
  year={2014},
  organization={IEEE}
}

@inproceedings{Barbieri2016,
  title={Design of cyber-physical systems: Definition and metamodel for reusable resources},
  author={Barbieri, Giacomo and Fantuzzi, Cesare},
  booktitle={2016 IEEE 21st International Conference on Emerging Technologies and Factory Automation (ETFA)},
  pages={1--9},
  year={2016},
  organization={IEEE}
}

@article{Chen2011,
  title={Petri net modeling of cyber-physical attacks on smart grid},
  author={Chen, Thomas M and Sanchez-Aarnoutse, Juan Carlos and Buford, John},
  journal={IEEE Transactions on Smart Grid},
  volume={2},
  number={4},
  pages={741--749},
  year={2011},
  publisher={IEEE}
}

@inproceedings{Jarus2016,
  title={Models, metamodels, and model transformation for cyber-physical systems},
  author={Jarus, Nathan and Sarvestani, Sahra Sedigh and Hurson, Ali R},
  booktitle={2016 Seventh International Green and Sustainable Computing Conference (IGSC)},
  pages={1--8},
  year={2016},
  organization={IEEE}
}

@inproceedings{Whalen2014,
  title={Structuring Simulink models for verification and reuse},
  author={Whalen, Michael W and Murugesan, Anitha and Rayadurgam, Sanjai and Heimdahl, Mats PE},
  booktitle={Proceedings of the 6th International Workshop on Modeling in Software Engineering},
  pages={19--24},
  year={2014},
  organization={ACM}
}

@article{Orojloo2017,
  title={A game-theoretic approach to model and quantify the security of cyber-physical systems},
  author={Orojloo, Hamed and Azgomi, Mohammad Abdollahi},
  journal={Computers in Industry},
  volume={88},
  pages={44--57},
  year={2017},
  publisher={Elsevier}
}

@article{Petnga2016,
  title={An ontological framework for knowledge modeling and decision support in cyber-physical systems},
  author={Petnga, Leonard and Austin, Mark},
  journal={Advanced Engineering Informatics},
  volume={30},
  number={1},
  pages={77--94},
  year={2016},
  publisher={Elsevier}
}

@article{Goncalves2016,
  title={Managing CPS complexity: Design method for Unmanned Aerial Vehicles},
  author={Gon{\c{c}}alves, Fernando S and Raffo, Guilherme V and Becker, Leandro B},
  journal={IFAC-PapersOnLine},
  volume={49},
  number={32},
  pages={141--146},
  year={2016},
  publisher={Elsevier}
}

@article{Feldmann2013,
  title={Model-driven engineering and semantic technologies for the design of cyber-physical systems},
  author={Feldmann, Stefan and R{\"o}sch, Susanne and Sch{\"u}tz, Daniel and Vogel-Heuser, Birgit},
  journal={IFAC Proceedings Volumes},
  volume={46},
  number={7},
  pages={210--215},
  year={2013},
  publisher={Elsevier}
}

@inproceedings{Cheng2014,
  title={Towards a stochastic occurrence-based modeling approach for stochastic cpss},
  author={Cheng, Bei and Du, Dehui},
  booktitle={2014 Theoretical Aspects of Software Engineering Conference},
  pages={162--169},
  year={2014},
  organization={IEEE}
}

@article{Xin2015,
  title={Cyber-physical modeling and cyber-contingency assessment of hierarchical control systems},
  author={Xin, Shujun and Guo, Qinglai and Sun, Hongbin and Zhang, Boming and Wang, Jianhui and Chen, Chen},
  journal={IEEE Transactions on Smart Grid},
  volume={6},
  number={5},
  pages={2375--2385},
  year={2015},
  publisher={IEEE}
}

@inproceedings{VanAcker2015,
  title={Managing heterogeneity in model-based systems engineering of cyber-physical systems},
  author={Van Acker, Bert and Denil, Joachim and Vangheluwe, Hans and De Meulenaere, Paul},
  booktitle={2015 10th International Conference on P2P, Parallel, Grid, Cloud and Internet Computing (3PGCIC)},
  pages={617--622},
  year={2015},
  organization={IEEE}
}

@inproceedings{Plasse2017,
  title={An adaptive modeling framework for bivariate data streams with applications to change detection in cyber-physical systems},
  author={Plasse, Joshua and Noble, Jordan and Myers, Kary},
  booktitle={2017 IEEE International Conference on Data Mining Workshops (ICDMW)},
  pages={1074--1081},
  year={2017},
  organization={IEEE}
}

@inproceedings{Brandenbourger2016,
  title={Behavior modeling of automation components using cross-domain interdependencies},
  author={Brandenbourger, Benjamin and Vathoopan, Milan and Zoitl, Alois},
  booktitle={2016 IEEE 21st International Conference on Emerging Technologies and Factory Automation (ETFA)},
  pages={1--4},
  year={2016},
  organization={IEEE}
}

@inproceedings{Irisarri2016,
  title={A model-based approach for process monitoring in oil production industry},
  author={Irisarri, Edurne and Garc{\'\i}a, Marcelo V and P{\'e}rez, Federico and Est{\'e}vez, Elisabet and Marcos, Marga},
  booktitle={2016 IEEE 21st International Conference on Emerging Technologies and Factory Automation (ETFA)},
  pages={1--4},
  year={2016},
  organization={IEEE}
}

@inproceedings{Yan2009,
  title={Integrated simulation and emulation platform for cyber-physical system security experimentation},
  author={Yan, Wei and Xue, Yuan and Li, Xiaowei and Weng, Jiannian and Busch, Timothy and Sztipanovits, Janos},
  booktitle={Proceedings of the 1st international conference on High Confidence Networked Systems},
  pages={81--88},
  year={2012},
  organization={ACM}
}

@article{Kuesap2008,
  title={Cps-based threat modeling for critical infrastructure protection},
  author={Ding, Jianguo and Atif, Yacine and Andler, Sten F and Lindstr{\"o}m, Birgitta and Jeusfeld, Manfred},
  journal={ACM SIGMETRICS Performance Evaluation Review},
  volume={45},
  number={2},
  pages={129--132},
  year={2017},
  publisher={ACM New York, NY, USA}
}

@inproceedings{Thramboulidis,
  title={Cyber-physical microservices: An IoT-based framework for manufacturing systems},
  author={Thramboulidis, Kleanthis and Vachtsevanou, Danai C and Solanos, Alexandros},
  booktitle={2018 IEEE Industrial Cyber-Physical Systems (ICPS)},
  pages={232--239},
  year={2018},
  organization={IEEE}
}

@article{SampathKumar2015,
  title={Unified meta-modeling framework using bond graph grammars for conceptual modeling},
  author={Kumar, Veera Ragavan Sampath and Shanmugavel, Madhavan and Ganapathy, Velappa and Shirinzadeh, Bijan},
  journal={Robotics and Autonomous Systems},
  volume={72},
  pages={114--130},
  year={2015},
  publisher={Elsevier}
}

@inproceedings{Nannapaneni2016,
  title={Towards reliability-based decision making in cyber-physical systems},
  author={Nannapaneni, Saideep and Mahadevan, Sankaran and Pradhan, Subhav and Dubey, Abhishek},
  booktitle={2016 IEEE International Conference on Smart Computing (SMARTCOMP)},
  pages={1--6},
  year={2016},
  organization={IEEE}
}

@inproceedings{Cohen2015,
  title={A credible autocoding application within a rocket and its payload},
  author={Cohen, Raphael and Long, Anh-Toan Bui and Jobredeaux, Romain and Feron, Eric},
  booktitle={2015 IEEE/AIAA 34th Digital Avionics Systems Conference (DASC)},
  pages={8C4--1},
  year={2015},
  organization={IEEE}
}

@inproceedings{Tan2013,
  title={Guaranteeing proper-temporal-embedding safety rules in wireless cps: A hybrid formal modeling approach},
  author={Tan, Feng and Wang, Yufei and Wang, Qixin and Bu, Lei and Zheng, Rong and Suri, Neeraj},
  booktitle={2013 43rd Annual IEEE/IFIP International Conference on Dependable Systems and Networks (DSN)},
  pages={1--12},
  year={2013},
  organization={IEEE}
}

@inproceedings{Koutsoumpas2015,
  title={A model-based approach for the specification of a virtual power plant operating in open context},
  author={Koutsoumpas, Vasileios},
  booktitle={Proceedings of the First International Workshop on Software Engineering for Smart Cyber-Physical Systems},
  pages={26--32},
  year={2015},
  organization={IEEE Press}
}

@inproceedings{Barve2018,
  title={Towards a Design Studio for Collaborative Modeling and Co-Simulations of Mixed Electrical Energy Systems},
  author={Barve, Yogesh and Neema, Himanshu and Rees, Stephen and Sztipanovits, Janos},
  booktitle={2018 IEEE International Science of Smart City Operations and Platforms Engineering in Partnership with Global City Teams Challenge (SCOPE-GCTC)},
  pages={24--29},
  year={2018},
  organization={IEEE}
}

@inproceedings{Pagliari2018,
  title={Multi-modeling approach to performance engineering of Cyber-Physical Systems design},
  author={Pagliari, Lorenzo and Mirandola, Raffaela and Trubiani, Catia},
  booktitle={2017 22nd International Conference on Engineering of Complex Computer Systems (ICECCS)},
  pages={142--145},
  year={2017},
  organization={IEEE}
}

@inproceedings{Palachi2013,
  title={Simulation of cyber physical models using SysML and numerical solvers},
  author={Palachi, Eldad and Cohen, Chaim and Takashi, Sakairi},
  booktitle={2013 IEEE International Systems Conference (SysCon)},
  pages={671--675},
  year={2013},
  organization={IEEE}
}

@inproceedings{Navet2016,
  title={CPAL: High-level abstractions for safe embedded systems},
  author={Navet, Nicolas and Fejoz, Lo{\"\i}c},
  booktitle={Proceedings of the International Workshop on Domain-Specific Modeling},
  pages={35--41},
  year={2016},
  organization={ACM}
}

@inproceedings{Bakirtzis2018,
  title={A model-based approach to security analysis for cyber-physical systems},
  author={Bakirtzis, Georgios and Carter, Bryan T and Elks, Carl R and Fleming, Cody H},
  booktitle={2018 Annual IEEE International Systems conference (SysCon)},
  pages={1--8},
  year={2018},
  organization={IEEE}
}

@inproceedings{Sinha2016,
  title={Requirements-aided automatic test case generation for industrial cyber-physical systems},
  author={Sinha, Roopak and Pang, Cheng and Mart{\'\i}nez, Gerardo Santill{\'a}n and Kuronen, Juha and Vyatkin, Valeriy},
  booktitle={2015 20th International Conference on Engineering of Complex Computer Systems (ICECCS)},
  pages={198--201},
  year={2015},
  organization={IEEE}
}

@inproceedings{Neema2018,
  title={Integrated simulation testbed for security and resilience of CPS},
  author={Neema, Himanshu and Potteiger, Bradley and Koutsoukos, Xenofon and Karsai, Gabor and Volgyesi, Peter and Sztipanovits, Janos},
  booktitle={Proceedings of the 33rd Annual ACM Symposium on Applied Computing},
  pages={368--374},
  year={2018},
  organization={ACM}
}

@article{Kacem2017,
  title={Application of a modeling approach on a cyber-physical system" RobAIR"},
  author={Kacem, Mohamed Amine Haj and Simeu-Abazi, Zineb and Gascard, Eric and Lemasson, Germain and Maisonnasse, J{\'e}r{\^o}ome},
  journal={IFAC-PapersOnLine},
  volume={50},
  number={1},
  pages={14230--14235},
  year={2017},
  publisher={Elsevier}
}

@inproceedings{Alshareef2018,
  title={Model-driven time-accurate DEVS-based approaches for CPS design},
  author={Alshareef, Abdurrahman and Sarjoughian, Hessam S},
  booktitle={Proceedings of the Model-driven Approaches for Simulation Engineering Symposium},
  pages={8},
  year={2018},
  organization={Society for Computer Simulation International}
}

@inproceedings{Rocchetto2017,
  title={Towards formal security analysis of industrial control systems},
  author={Rocchetto, Marco and Tippenhauer, Nils Ole},
  booktitle={Proceedings of the 2017 ACM on Asia Conference on Computer and Communications Security},
  pages={114--126},
  year={2017},
  organization={ACM}
}

@inproceedings{Rashid2018,
  title={Modeling and simulation of cyberattacks for resilient cyber-physical systems},
  author={Rashid, Nafiul and Wan, Jiang and Quiros, Gustavo and Canedo, Arquimedes and Al Faruque, Mohammad Abdullah},
  booktitle={2017 13th IEEE Conference on Automation Science and Engineering (CASE)},
  pages={988--993},
  year={2017},
  organization={IEEE}
}

@inproceedings{Low2017,
  title={High assurance code generation for cyber-physical systems},
  author={Low, Tze Meng and Franchetti, Franz},
  booktitle={2017 IEEE 18th International Symposium on High Assurance Systems Engineering (HASE)},
  pages={104--111},
  year={2017},
  organization={IEEE}
}

@inproceedings{Broenink2016,
  title={A co-design approach for embedded control software of cyber-physical systems},
  author={Broenink, Jan F and Vos, Peter-Jan D and Lu, Zhou and Bezemer, Maarten M},
  booktitle={2016 11th System of Systems Engineering Conference (SoSE)},
  pages={1--5},
  year={2016},
  organization={IEEE}
}

@article{Morozov2018,
  title={Multi-paradigm modelling of Cyber-Physical Systems},
  author={Morozov, Dmitry and Lezoche, Mario and Panetto, Herv{\'e}},
  journal={IFAC-PapersOnLine},
  volume={51},
  number={11},
  pages={1385--1390},
  year={2018},
  publisher={Elsevier}
}

@article{Hahn2015,
  title={A multi-layered and kill-chain based security analysis framework for cyber-physical systems},
  author={Hahn, Adam and Thomas, Roshan K and Lozano, Ivan and Cardenas, Alvaro},
  journal={International Journal of Critical Infrastructure Protection},
  volume={11},
  pages={39--50},
  year={2015},
  publisher={Elsevier}
}

@inproceedings{Zhang2011,
  title={Aspect-oriented mda approach for non-functional properties of distributed cyber physical systems},
  author={Zhang, Lichen},
  booktitle={2011 10th International Symposium on Distributed Computing and Applications to Business, Engineering and Science},
  pages={284--288},
  year={2011},
  organization={IEEE}
}

@inproceedings{Reijnen2017,
  title={Supervisory control synthesis for a waterway lock},
  author={Reijnen, FFH and Goorden, MA and van de Mortel-Fronczak, JM and Rooda, JE},
  booktitle={2017 IEEE Conference on Control Technology and Applications (CCTA)},
  pages={1562--1563},
  year={2017},
  organization={IEEE}
}

@inproceedings{Pohlmann2014,
  title={Application of an intelligent network architecture on a cooperative cyber-physical system: An experience report},
  author={Pohlmann, Uwe and Trsek, Henning and D{\"u}rkop, Lars and Dziwok, Stefan and Oesters{\"o}tebier, Felix},
  booktitle={Proceedings of the 2014 IEEE Emerging Technology and Factory Automation (ETFA)},
  pages={1--6},
  year={2014},
  organization={IEEE}
}

@article{Blackburn2014,
  title={Virtual design and verification of cyber-physical systems: Industrial process plant design},
  author={Blackburn, Mark and Denno, Peter},
  journal={Procedia Computer Science},
  volume={28},
  pages={883--890},
  year={2014},
  publisher={Elsevier}
}

@inproceedings{Passarini2014,
  title={The assisted transformation of models: Supporting cyber-physical systems design by extracting architectural aspects and operating modes from simulink functional models},
  author={Passarini, Rosane F{\'a}tima and Becker, Leandro Buss and Farines, Jean-Marie},
  booktitle={2013 III Brazilian Symposium on Computing Systems Engineering},
  pages={47--52},
  year={2013},
  organization={IEEE}
}

@inproceedings{Silva2014,
  title={A model-based architecture for testing medical cyber-physical systems},
  author={Silva, Lenardo C and Perkusich, Mirko and Bublitz, Frederico M and Almeida, Hyggo O and Perkusich, Angelo},
  booktitle={Proceedings of the 29th Annual ACM Symposium on Applied Computing},
  pages={25--30},
  year={2014},
  organization={ACM}
}

@inproceedings{Hu2013,
  title={Dependability Modelling and Evaluation of Cyber-Physical Systems: A Model-Driven Perspective},
  author={Hu, Xiaojing and Liu, Shixi and Chen, Guilin and Jiang, Cuiqing},
  booktitle={1st International Workshop on Cloud Computing and Information Security},
  year={2013},
  organization={Atlantis Press}
}

@inproceedings{Pradhan2015,
  title={Chariot: A domain specific language for extensible cyber-physical systems},
  author={Pradhan, Subhav M and Dubey, Abhishek and Gokhale, Aniruddha and Lehofer, Martin},
  booktitle={Proceedings of the workshop on domain-specific modeling},
  pages={9--16},
  year={2015},
  organization={ACM}
}

@inproceedings{Zhao2017,
  title={Multi-View Design for Cyber-Physical Systems},
  author={Zhao, Hui and Apvrille, Ludovic and Mallet, Fr{\'e}d{\'e}ric},
  year={2017}
}

@article{Lezoche2018,
  title={Cyber-Physical Systems, a new formal paradigm to model redundancy and resiliency},
  author={Lezoche, Mario and Panetto, Herv{\'e}},
  journal={Enterprise Information Systems},
  pages={1--22},
  year={2018},
  publisher={Taylor \& Francis}
}

@article{Heinzemann2017slrcps,
  title={Transactional execution of hierarchical reconfigurations in cyber-physical systems},
  author={Heinzemann, Christian and Becker, Steffen and Volk, Andreas},
  journal={Software \& Systems Modeling},
  volume={18},
  number={1},
  pages={157--189},
  year={2019},
  publisher={Springer}
}

@inproceedings{Cicirelli2018,
  title={A metamodel framework for edge-based smart environments},
  author={Cicirelli, Franco and Fortino, Giancarlo and Guerrieri, Antonio and Mercuri, Alessandro and Spezzano, Giandomenico and Vinci, Andrea},
  booktitle={2018 IEEE International Conference on Cloud Engineering (IC2E)},
  pages={286--291},
  year={2018},
  organization={IEEE}
}

@article{Fan2018,
  title={A simulation platform for human-machine interaction safety analysis of cyber-physical systems},
  author={Fan, Chin-Feng and Chan, Ching-Chieh and Yu, Hsiang-Yu and Yih, Swu},
  journal={International journal of industrial ergonomics},
  volume={68},
  pages={89--100},
  year={2018},
  publisher={Elsevier}
}

@inproceedings{Cheng2015,
  title={Modana: An integrated framework for modeling and analysis of energy-aware CPSs},
  author={Cheng, Bei and Wang, Xiao and Liu, Jufu and Du, Dehui},
  booktitle={2015 IEEE 39th Annual Computer Software and Applications Conference},
  volume={2},
  pages={127--136},
  year={2015},
  organization={IEEE}
}

@inproceedings{Chen2018,
  title={Ontology Based Behavior Verification for Complex Systems},
  author={Chen, Ruirui and Liu, Yusheng and Ye, Xiaoping},
  booktitle={ASME 2018 International Design Engineering Technical Conferences and Computers and Information in Engineering Conference},
  year={2018},
  organization={American Society of Mechanical Engineers Digital Collection}
}

@incollection{Murugesan,
  title={From requirements to code: Model based development of a medical cyber physical system},
  author={Murugesan, Anitha and Heimdahl, Mats PE and Whalen, Michael W and Rayadurgam, Sanjai and Komp, John and Duan, Lian and Kim, Baek-Gyu and Sokolsky, Oleg and Lee, Insup},
  booktitle={Software Engineering in Health Care},
  pages={96--112},
  year={2014},
  publisher={Springer}
}

@inproceedings{B2018,
  title={Verification of the consistency of time-aware cyber-physical processes},
  author={Graja, Imen and Kallel, Slim and Guermouche, Nawal and Kacem, Ahmed Hadj},
  booktitle={International Conference on Service-Oriented Computing},
  pages={67--79},
  year={2017},
  organization={Springer}
}

@inproceedings{Graja,
  title={BPMN4CPS: A BPMN extension for modeling cyber-physical systems},
  author={Graja, Imen and Kallel, Slim and Guermouche, Nawal and Kacem, Ahmed Hadj},
  booktitle={2016 IEEE 25th International Conference on Enabling Technologies: Infrastructure for Collaborative Enterprises (WETICE)},
  pages={152--157},
  year={2016},
  organization={IEEE}
}

@article{Ali2018,
  title={Failure Detection and Prevention for Cyber-Physical Systems Using Ontology-Based Knowledge Base},
  author={Ali, Nazakat and Hong, Jang-Eui},
  journal={Computers},
  volume={7},
  number={4},
  pages={68},
  year={2018},
  publisher={Multidisciplinary Digital Publishing Institute}
}

@inproceedings{Guan2018,
  title={xSHS: An Executable Domain-Specific Modeling Language for Modeling Stochastic and Hybrid Behaviors of Cyber-Physical Systems},
  author={Guan, Chunlin and Ao, Yi and Du, Dehui and Mallet, Fr{\'e}d{\'e}ric},
  booktitle={2018 25th Asia-Pacific Software Engineering Conference (APSEC)},
  pages={683--687},
  year={2018},
  organization={IEEE}
}


